Finding Effective Geo-Social Group for Impromptu Activity with Multiple Demands

Geo-social group search aims to find a group of people proximate to a location while socially related. One of the driven applications for geo-social group search is organizing an impromptu activity. This is because the social cohesiveness of a found geo-social group ensures a good communication atmosphere and the spatial closeness of the geo-social group reduces the preparation time for the activity. Most existing works treat geo-social group search as a problem that finds a group satisfying a single social constraint while optimizing the spatial proximity. However, when an impromptu activity has additional demands on attendees, e.g., the activity requires that the attendees have certain set of skills, the existing works cannot find an effective geo-social group efficiently. In this paper, we study how to find a group that is most proximate to a query location while satisfying multiple constraints. Specifically, the multiple constraints on which we focus include social constraint, size constraint and keyword constraint. We propose a novel search framework which first effectively narrows down the search space with theoretical guarantees and then efficiently finds the optimum result. Although our model considers multiple constraints, novel techniques devised in this paper ensure that search cost is equivalent to parameterized constant times of one time social constraint checking on a vastly restricted search space. We conduct extensive experiments on both real and semi-synthetic datasets for demonstrating the efficiency of the proposed search algorithm. To evaluate the effectiveness, we conduct two case studies on real datasets, demonstrating the superiority of our proposed model.

==> AlgInsideATruss.tex <==














%\noindent\textbf{Incremental $(\rho, t)$-truss checking}.

%  every connected subgraph satisfying keyword constraint. For other part of subgraphs, we would not apply $(\rho, t)$-truss checking until





%Below, we use $\mathcal{A}$ to denote the structure for local exploration.

%\noindent\textbf{Complete expanding stage}. With expanding strategy and the local exploration data structure, we are ready to show a complete expanding stage. Initially, we build $\mathcal{A}$ for a maximal connected $(\rho,t)$-truss. Then, the initial exploration boundary is set to be the location of the e



%Mathematically, we shall have a function that could result a series of distances $\{d_{1},\ldots, d_(s)\}$. such that for any successive $d_{i}$, $d_{i+1}$ ($i$ $>$ $1$ and $i$ $<$ $s$) $d_{i}\leq d_{i+1}$ shall hold.
%Particular, we propose that for any successive $d_{i}$, $d_{i+1}$ ($i$ $>$ $1$ and $i$ $<$ $s$), $d_{i}$ and $d_{j}$ shall follow the %invariant below, denoted as $\Delta$ size invariant.






%Since maximal ($\rho$, $t$)-trusses have no overlaps and the total number of the maximal ($\rho$, $t$)-trusses is low



%\noindent\textbf{Pruning over maximal ($\rho$, $t$)-trusses}. Given two maximal ($\rho$, $t$)-trusses $S$ and $S^{\prime}$, let $d_{min}$ be $min$$\{||\lambda -v || v\in S  \}$ ($d_{min}^{\prime}$ $=$ $min$$\{||\lambda -v || v\in S  \}$), if $DIST(\lambda,S)\le d_{min}^{\prime}$, we can safely ignore $S^{\prime}$. 

==> problemhardness.tex <==
\iffalse
\section{Hardness Analysis}

\begin{theorem}
	
\end{theorem}
\begin{algorithm}
	determine $c^{*}$\;
	$d^{*}$ $\leftarrow$ $\infty$\; 
	$S^{*}\leftarrow \emptyset$\; 
	\ForEach{$d$ $\in$ $\{dist(v,\lambda)|v\in V(G)\}$ }{
		let $G_{\leq d}$ be the subgraph of $G$ located in the cycle $cycle(\lambda, d)$\;
		$S$ $\leftarrow$ $(\rho, c^{*})$-truss in $G_{\leq d}$\;
		\If{$S$ $\ne$ $\emptyset$ $\&\&$ $dist(S^{*},\lambda)$ $<$ $d^{*}$}{
			$S^{*}$ $\leftarrow$ $S$\;
		}
	}
	\Return $S^{*}$
	\caption{Polynomial procedure}
\end{algorithm}


\begin{algorithm}
	\KwIn{$\qk$,$G$ with truss index} 
	\KwOut{$c^{*}$}
	\For{$c$ $\leftarrow$ $c_{max}$ \textup{\textbf{to}} 1}{
		\If{\textup{ if there is a $(\rho, c)$-truss}}{
			$c^{*}\leftarrow c$\;
			\Return{$c^{*}$}\;
		}
	}
	\caption{Determine $c^{*}$}
\end{algorithm}


\begin{algorithm}
	\KwIn{$\qk$, $G$, $k$, $\rho$}
	\KwOut{$(\rho, k)$-truss or $\emptyset$}
	\ForEach{maximal connected k-truss $T$ $\in G$}{
		$mink^{*} \leftarrow \infty$\;
		\ForEach{$k$ $\in$ $\qk$}{
			$mink$ $\leftarrow$  the number of vertices containing $k$\; 
			\If{$mink$ $<$ $mink^{*}$}{
				$mink^{*} \leftarrow mink$\;
			}
		}
		\If{$mink^{*}\geq \rho$ }{
			\Return $T$ as $(\rho, k)$-truss  \; 
		}		
	}
	\Return $\emptyset$\;
	\caption{Compute a $(\rho, k)$-truss}
\end{algorithm}
\fi


